In-Context Learning with Noisy Labels

In-context learning refers to the emerging ability of large language models (LLMs) to perform a target task without additional training, utilizing demonstrations of the task. Recent studies aim to enhance in-context learning performance by selecting more useful demonstrations. However, they overlook the presence of inevitable noisy labels in task demonstrations that arise during the labeling process in the real-world. In this paper, we propose a new task, in-context learning with noisy labels, which aims to solve real-world problems for in-context learning where labels in task demonstrations would be corrupted. Moreover, we propose a new method and baseline methods for the new task, inspired by studies in learning with noisy labels. Through experiments, we demonstrate that our proposed method can serve as a safeguard against performance degradation in in-context learning caused by noisy labels.

==> Algorithms/1_reward_calculation.tex <==
% \begin{algorithm}[!h]
% \footnotesize
% \begin{algorithmic}[1]
% \State {\bfseries Input:} vision-language model, text-to-image model, grounding model, similarity model, input image \\

% \State {\bfseries Output:} reward value \\

% \State Process input image through vision-language model to produce detailed caption

% \State Process text output through text-to-image model to obtain reconstructed image

% \State Initialize penalty values: $\textit{penalty}_1 = 0$, $\textit{penalty}_2 = 0$, $\textit{penalty}_3 = 0$ \\

% \State {\textit{- Non-existent Objects Penalty -}}
% \State Find objects matched only in the reconstructed image using grounding model, denote as $N$
% \State Calculate $\textit{penalty}_1$: decrease penalty by 1 for each object in $N$ \\

% \State {\textit{- Unfaithful Object Attributes Penalty -}}
% \State Find object-region pairs matched in both input and reconstructed image using grounding model, denote as $M$
% \State Calculate $\textit{penalty}_2$: for each object pair $o_i$ and $o_j$ in $M$, add $(1 - \textit{sim}_i)$, where $\textit{sim}_i$ is the similarity score computed using similarity model \\

% \State {\textit{- Inaccurate Relationships Penalty -}}
% \State Calculate similarity score $\textit{sim}_{whole}$ between input and reconstructed image using similarity model
% \State Set $\textit{penalty}3 = 1 - \textit{sim}{whole}$ \\

% \State {\textit{- Overall Reward Calculation -}}
% \State Initialize reward value $\textit{reward} = 0$
% \State Calculate reward as the sum of the penalties: $\textit{reward} = \textit{penalty}_1 + \textit{penalty}_2 + \textit{penalty}_3$

% \State Return $\textit{reward}$

% \caption{Reward Calculation}
% \label{alg:reward_calculation}
% \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}[!h]
% \footnotesize
% \begin{algorithmic}[1]
% \REQUIRE T2I: Text-to-Image Model, $G$: grounding model, CLIP: similarity model
% \REQUIRE $I$: Input image, $\{t_i\}_{i=1}^T$: Generated caption from the image

% % \STATE I_rec = T2I($I$)
% \FOR{${i=1}$ to $T$}
%     \STATE $p_{{H1}, t} = 0$
%     \STATE $p_{{H2}, t} = 0$
% \ENDFOR
% \STATE $I_{rec} \leftarrow \textrm{T2I}(\{t_i\}_{i=1}^T)$
% \STATE $\{(t_{{s_j}..{e_j}}, I_{rec}^j)\}_{j=1}^N$ $\leftarrow$ $G(\{t_i\}_{i=1}^T, I_{rec})$
% \FOR{${j=1}$ to $N$}
%     \STATE $(t_{{s^\prime_j}..{e^\prime_j}}, I^j)$ $\leftarrow$ $G(\{t_{{s_j}..{e_j}}\}, I)$
%     \IF{$(t_{{s^\prime_j}..{e^\prime_j}}, I^j) = \emptyset$}
%         \STATE $p_{{H1}, e_j} = -1$
%     \ELSE %\IF{$t_{{s^\prime_j}..{e^\prime_j}} \cap t_{{s_j}..{e_j}} \ne \emptyset$}
%         \STATE $p_{{H2}, e_j} = \textrm{CLIP}(I^j, I_{rec}^j)$
%     \ENDIF
% \ENDFOR
% \STATE $p_{H3} = -\textrm{CLIP}(I, I_{rec})$

% \caption{Reward Calculation}
% \label{alg:reward_calculation}
% \end{algorithmic}
% \end{algorithm}

\begin{algorithm}[!h]
\footnotesize
\begin{algorithmic}[1]
\REQUIRE T2I: Text-to-Image Model, $G$: grounding model, CLIP: similarity model
\REQUIRE $\textrm{I}$: Input image, $s_{1..T}$: Generated caption from the image

\STATE Initialize $p_{{\textrm{H1}}, t}$ and $p_{{\textrm{H1}}, t}$ to 0 for $t = 1$ to $T$
% \FOR{${i=1}$ to $T$}
%     \STATE $p_{{H1}, t} = 0$ \hfill $\leftarrow$ Initialize penalty for H1
%     \STATE $p_{{H2}, t} = 0$ \hfill $\leftarrow$ Initialize penalty for H2
% \ENDFOR
\STATE $\textrm{I}_{rec} \leftarrow \textrm{T2I}(s_{1..T})$ % \hfill $\leftarrow$ Reconstruct image from text
\STATE $\{(s_{{b_j}..{e_j}}, \textrm{I}_{rec}^j)\}_{j=1}^N$ $\leftarrow$ $G(s_{1..T}, \textrm{I}_{rec})$  % \hfill $\leftarrow$ Grounding on reconstructed image and get object-region pairs
\STATE{Loop over object-region pairs in a batched manner:}
\FOR{${j=1}$ to $N$}
    \STATE $(s_{{b^\prime_j}..{e^\prime_j}}, \textrm{I}^j)$ $\leftarrow$ $G(\{s_{{b_j}..{e_j}}\}, \textrm{I})$ % \hfill $\leftarrow$ Grounding on original image
    \IF{$(s_{{b^\prime_j}..{e^\prime_j}}, \textrm{I}^j) = \emptyset$}
        \STATE $p_{\textrm{H1}, e_j} = -1$ \hfill $\leftarrow$ Penalty for non-existent objects
    \ELSE
        \STATE $p_{\textrm{H2}, e_j} = (1 - \textrm{CLIP}(\textrm{I}^j, \textrm{I}_{rec}^j))/2$ \hfill $\leftarrow$ Penalty for unfaithful object attributes
    \ENDIF
\ENDFOR
\STATE $p_{rec} = - \textrm{CLIP}(\textrm{I}, \textrm{I}_{rec})$ \hfill $\leftarrow$ Penalty for overall reconstruction

\caption{Reward Calculation}
\label{alg:reward_calculation}
\end{algorithmic}
\end{algorithm}


==> Algorithms/2_ppo_training.tex <==
% \begin{algorithm}[!h]
% \footnotesize
% \begin{algorithmic}[1]
% \State {\bfseries Input:} state observation function $g$, policy $\pi_\theta$, value function $V_\phi$, PPO clipping parameter $\epsilon$, step size $\alpha$, number of epochs $E$, batch size $B$ \\
% \State {\bfseries Output:} the trained policy $\pi_\theta$ and value function $V_\phi$ \\
% \State {\textit{- PPO Training -}}
% \Repeat
% \State Observe the state $s_t$ using the state observation function $g$
% \State Sample action $a_t \sim \pi_\theta(a|s_t)$
% \State Execute $a_t$ and observe the next state $s_{t+1}$ and immediate reward $r_t$
% \State Store the transition $(s_t, a_t, r_t, s_{t+1})$ into buffer $B$
% \If{buffer $B$ is full}
% \For{epoch $i = 1, \dots, E$}
% \State Sample a minibatch of transitions $(s, a, r, s')$ from buffer $B$
% \State Compute advantages $A(s, a)$ using Generalized Advantage Estimation (GAE)
% \State Update policy $\pi_\theta$ and value function $V_\phi$ using the Proximal Policy Optimization (PPO) objective
% \State $\theta \leftarrow \theta + \alpha \nabla_\theta J(\theta)$
% \State $\phi \leftarrow \phi + \alpha \nabla_\phi J(\phi)$
% \EndFor
% \State Empty the buffer $B$
% \EndIf
% \Until{desired performance reached or maximum training time reached}

% \caption{PPO Training}
% \label{alg:2_ppo_training}
% \end{algorithmic}
% \end{algorithm}



\begin{algorithm}[!h]
\footnotesize
\begin{algorithmic}[1]
% \State {\bfseries Input:} 
\REQUIRE policy $\pi_\theta$, reference policy $\pi_{\text{ref}}$, value model $V_\phi$, reward model $r$, PPO clipping parameter $\epsilon$, step size $\alpha$, number of epochs $E$, batch size ${B}$, image dataset $\mathcal{D}$, hallucination penalty weights $w_{H1}, w_{H2}, w_{H3}$, KLD scaling parameter $\beta$
% \State {\bfseries Output:} the trained policy $\pi_\theta$ % and value function $V_\phi$ 
\REPEAT
\STATE Sample batch $\{x_i\}_{i=1}^B \sim \mathcal{D}$ with batch size ${B}$
\STATE Sample output sequence $s^i_{1..T} \sim p_\theta(s_{1..T}|x_i)$ for each of the data $x_i$ in batch
\STATE Compute rewards $r^i_{1..T}$ using reward model $ r(x_i, s^i_{1..T}$ for each output sequence
\STATE Compute advantages $A^i_{1..T}$ using Generalized Advantage Estimation (GAE):
\STATE \quad $\delta^i_t = r^i_{t} + \gamma V_\phi(s^i_{t+1}) - V_\phi(s^i_t)$
\STATE \quad $A^i_t = \delta^i_t + (\gamma \lambda) \delta^i_{t+1} + \cdots + (\gamma \lambda)^{T-t+1} \delta^i_{T-1}$
\STATE Compute value targets $V^i_{t=1..T}$ with $V^i_t = \sum_{t^\prime=t}^T r^i_t$
\FOR{PPO epoch $i = 1, \dots, E$}
    % \STATE Update policy $\pi_\theta$ and value function $V_\phi$ using the PPO objective:
    \STATE Update policy $\pi_\theta$ using the clipped surrogate objective:
    \STATE \quad $\theta \leftarrow \arg \max_\theta \frac{1}{{B}} \sum_{i=1}^{{B}} \left[ \frac{1}{T} \sum_{t=1}^{T} \min\left(\frac{p_\theta}{p_{\theta_{old}}} A_t^i, \right. \right.$
\STATE \quad \quad \quad \quad $\left. \left. \text{clip}\left(\frac{p_\theta}{p_{\theta_{old}}}, 1-\epsilon, 1+\epsilon\right) A_t^i\right) \right]$
    % \STATE \quad $\theta \leftarrow \arg \max_\theta \frac{1}{B} \sum_{i=1}^{B} \frac{1}{T} \sum_{t=1}^{T} \min(\frac{p_\theta}{p_{\theta_{old}}} A_t^i, \text{clip}(\frac{p_\theta}{p_{\theta_{old}}}, 1-\epsilon, 1+\epsilon) A_t^i)$
    \STATE Update value model $V_\phi$ using L2 loss:
    \STATE \quad $L^{VF}(\phi) = \sum_{i=1}^{{B}} \sum_{t=1}^{T} \left( V_\phi(s_t^i) - V_t^i \right)^2$

    % \State \quad $L^{VF}(\phi) = \mathbb{E}_{t} \left[ (V_\phi(s_t) - V^i_t)^2 \right]$
\ENDFOR
    % \State \quad minimize $\mathbb{E}{x \sim D, y \sim \pi{\theta}(y|x)} \left[ r(\tau) - \beta \log \frac{\pi_{\theta}(y|x)}{\pi_{\text{ref}}(y|x)} \right]$
    % \State $\theta \leftarrow \theta + \alpha \nabla_\theta J(\theta)$
    % \State $\phi \leftarrow \phi + \alpha \nabla_\phi J(\phi)$
\UNTIL{maximum iteration reached}

\caption{PPO Training with Fine-grained Rewards}
\label{alg:modified_ppo_training}
\end{algorithmic}
\end{algorithm}

==> Figures/3_stability.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{Figures/3_stability.pdf}
    \caption{Stability of the rectification method.}
    \vspace{-1em}
    \label{fig:3_stability}
\end{figure}

==> Tables/2_llm_result.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\caption{Experimental results on Llama2-7B and Mistral-7B-v0.1.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|c|c|cccccc|cccccc|cccccc}
\hline
\multirow{2}{*}{Model} &
  \multirow{2}{*}{Retriever} &
  \multirow{2}{*}{Method} &
  \multicolumn{6}{c|}{MRPC} &
  \multicolumn{6}{c|}{SST-5} &
  \multicolumn{6}{c}{Tweet} \\
 &
   &
   &
  0 &
  0.1 &
  0.2 &
  0.3 &
  0.4 &
  0.5 &
  0 &
  0.1 &
  0.2 &
  0.3 &
  0.4 &
  0.5 &
  0 &
  0.1 &
  0.2 &
  0.3 &
  0.4 &
  0.5 \\ \hline
\multirow{6}{*}{Llama2-7B} &
  \multirow{3}{*}{EPR} &
  w/o manipulation &
  77.7 &
  75.5 &
  76.5 &
  74.3 &
  62.3 &
  62.3 &
  50.2 &
  49.3 &
  \textbf{51.0} &
  47.6 &
  45.3 &
  45.4 &
  \textbf{59.5} &
  \textbf{61.5} &
  58.6 &
  60.0 &
  57.5 &
  52.9 \\ \cline{3-21} 
 &
   &
  correction &
  \multicolumn{6}{c|}{72.5 / 75.2*} &
  \multicolumn{6}{c|}{43.7 / 44.4*} &
  \multicolumn{6}{c}{57.3 / 57.3*} \\ \cline{3-21} 
 &
   &
  Rectification &
  \textbf{78.2} &
  \textbf{78.4} &
  \textbf{78.4} &
  \textbf{78.4} &
  \textbf{76.7} &
  \textbf{75.8} &
  \textbf{50.3} &
  \textbf{50.5} &
  50.3 &
  \textbf{50.2} &
  \textbf{50.6} &
  \textbf{49.4} &
  59.9 &
  59.8 &
  \textbf{59.9} &
  \textbf{59.6} &
  \textbf{60.3} &
  \textbf{59.4} \\ \cline{2-21} 
 &
  \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}TopK-\\ BERT\end{tabular}} &
  w/o manipulation &
  70.3 &
  70.6 &
  69.1 &
  66.9 &
  59.1 &
  60.0 &
  49.8 &
  47.2 &
  49.0 &
  47.3 &
  43.5 &
  40.4 &
  71.4 &
  69.7 &
  67.5 &
  64.7 &
  56.9 &
  55.8 \\ \cline{3-21} 
 &
   &
  correction &
  \multicolumn{6}{c|}{69.6 / 69.6*} &
  \multicolumn{6}{c|}{46.3 / 45.5*} &
  \multicolumn{6}{c}{57.4 / 60.0*} \\ \cline{3-21} 
 &
   &
  Rectification &
  \textbf{73.5} &
  \textbf{71.6} &
  \textbf{72.3} &
  \textbf{70.6} &
  \textbf{71.3} &
  \textbf{71.1} &
  \textbf{51.2} &
  \textbf{50.8} &
  \textbf{51.1} &
  \textbf{50.2} &
  \textbf{50.6} &
  \textbf{49.4} &
  \textbf{71.7} &
  \textbf{71.7} &
  \textbf{71.3} &
  \textbf{69.7} &
  \textbf{71.3} &
  \textbf{70.3} \\ \hline
\multirow{6}{*}{Mistral-7B} &
  \multirow{3}{*}{EPR} &
  w/o manipulation &
  77.7 &
  77.0 &
  76.5 &
  76.7 &
  61.3 &
  64.0 &
  \textbf{51.9} &
  \textbf{50.1} &
  48.5 &
  45.5 &
  44.3 &
  40.0 &
  \textbf{66.3} &
  \textbf{68.2} &
  63.3 &
  65.1 &
  61.8 &
  55.8 \\ \cline{3-21} 
 &
   &
  correction &
  \multicolumn{6}{c|}{74.5 / 76.0*} &
  \multicolumn{6}{c|}{44.8 / 42.6*} &
  \multicolumn{6}{c}{57.3 / 58.9*} \\ \cline{3-21} 
 &
   &
  Rectification &
  \textbf{78.4} &
  \textbf{77.9} &
  \textbf{77.9} &
  \textbf{78.9} &
  \textbf{77.0} &
  \textbf{77.0} &
  49.4 &
  49.9 &
  \textbf{49.5} &
  \textbf{49.9} &
  \textbf{49.8} &
  \textbf{49.8} &
  66.0 &
  65.8 &
  \textbf{65.8} &
  \textbf{65.8} &
  \textbf{65.8} &
  \textbf{65.8} \\ \cline{2-21} 
 &
  \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}TopK-\\ BERT\end{tabular}} &
  w/o manipulation &
  72.3 &
  72.1 &
  70.3 &
  67.9 &
  62.3 &
  62.3 &
  47.7 &
  46.4 &
  44.8 &
  42.7 &
  40.3 &
  39.2 &
  \textbf{74.6} &
  \textbf{71.5} &
  67.5 &
  65.9 &
  57.5 &
  57.5 \\ \cline{3-21} 
 &
   &
  correction &
  \multicolumn{6}{c|}{71.6 / 71.0*} &
  \multicolumn{6}{c|}{43.6 / 43.7*} &
  \multicolumn{6}{c}{57.2 / 59.5*} \\ \cline{3-21} 
 &
   &
  Rectification &
  \textbf{73.0} &
  \textbf{72.3} &
  \textbf{72.5} &
  \textbf{71.8} &
  \textbf{71.8} &
  \textbf{71.6} &
  \textbf{49.0} &
  \textbf{48.7} &
  \textbf{49.7} &
  \textbf{49.1} &
  \textbf{50.2} &
  \textbf{48.4} &
  72.1 &
  \textbf{71.5} &
  \textbf{71.4} &
  \textbf{70.2} &
  \textbf{70.3} &
  \textbf{69.1} \\ \hline
\end{tabular}
}
\label{tab:2_llm_result}
\end{table*}

==> Tables/old_baseline_result.tex <==
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|c|ccccc}
\hline
\multirow{2}{*}{Dataset} &
  \multirow{2}{*}{Method} &
  \multicolumn{5}{c}{Noise rates ($r$)} \\ \cline{3-7} 
 &
   &
  \multicolumn{1}{c|}{0} &
  \multicolumn{1}{c|}{0.1} &
  \multicolumn{1}{c|}{0.2} &
  \multicolumn{1}{c|}{0.3} &
  0.5 \\ \hline
\multirow{5}{*}{MRPC} &
  No correction &
  \multicolumn{1}{c|}{77.45} &
  \multicolumn{1}{c|}{75.49} &
  \multicolumn{1}{c|}{72.3} &
  \multicolumn{1}{c|}{66.18} &
  56.86 \\
 &
  Correction &
  \multicolumn{1}{c|}{77.45} &
  \multicolumn{1}{c|}{77.45} &
  \multicolumn{1}{c|}{77.45} &
  \multicolumn{1}{c|}{77.45} &
  77.45 \\
 &
  Weighting &
  \multicolumn{1}{c|}{77.45} &
  \multicolumn{1}{c|}{75.49} &
  \multicolumn{1}{c|}{71.81} &
  \multicolumn{1}{c|}{66.67} &
  55.88 \\
 &
  Reordering &
  \multicolumn{1}{c|}{76.96} &
  \multicolumn{1}{c|}{77.21} &
  \multicolumn{1}{c|}{75.98} &
  \multicolumn{1}{c|}{75} &
  74.51 \\
 &
  Selection &
  \multicolumn{1}{c|}{77.21} &
  \multicolumn{1}{c|}{77.21} &
  \multicolumn{1}{c|}{76.96} &
  \multicolumn{1}{c|}{77.45} &
  78.68 \\ \hline
\multirow{5}{*}{SST-5} &
  No correction &
  \multicolumn{1}{c|}{46.41} &
  \multicolumn{1}{c|}{42.6} &
  \multicolumn{1}{c|}{41.6} &
  \multicolumn{1}{c|}{37.69} &
  29.79 \\
 &
  Correction &
  \multicolumn{1}{c|}{45.23} &
  \multicolumn{1}{c|}{45.23} &
  \multicolumn{1}{c|}{45.23} &
  \multicolumn{1}{c|}{45.23} &
  45.23 \\
 &
  Weighting &
  \multicolumn{1}{c|}{46.41} &
  \multicolumn{1}{c|}{43.6} &
  \multicolumn{1}{c|}{40.78} &
  \multicolumn{1}{c|}{37.24} &
  32.33 \\
 &
  Reordering &
  \multicolumn{1}{c|}{46.13} &
  \multicolumn{1}{c|}{42.96} &
  \multicolumn{1}{c|}{46.41} &
  \multicolumn{1}{c|}{42.87} &
  39.96 \\
 &
  Selection &
  \multicolumn{1}{c|}{46.59} &
  \multicolumn{1}{c|}{45.05} &
  \multicolumn{1}{c|}{44.78} &
  \multicolumn{1}{c|}{45.32} &
  41.69 \\ \hline
\end{tabular}%
}
\caption{Results of baseline methods on GPT-Neo 2.7B as the inference model.}
\end{table}

==> Tables/old_compare.tex <==
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}ccccccc@{}}
\toprule
Dataset               & Method                             & 0     & 0.1   & 0.2   & 0.3   & 0.5   \\ \midrule
\multicolumn{1}{c|}{\multirow{2}{*}{MRPC}} & \multicolumn{1}{c|}{Correction} & 74.51 & 74.51 & 74.51 & 74.51 & 74.51 \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Rectification} & 75.49 & 75.98 & 76.47 & 75    & 74.51 \\ \midrule
\multicolumn{1}{c|}{\multirow{2}{*}{SST5}} & \multicolumn{1}{c|}{Correction} & 41.6  & 41.6  & 41.6  & 41.6  & 41.6  \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Rectification} & 47.27 & 46.18 & 46.18 & 46.73 & 45.64 \\ \bottomrule
\end{tabular}%
}
\caption{Comparison between the classifier-based correction and the rectifying network. GPT-Neo 2.7B and EPR are used for the inference model and the retriever, respectively.}
\end{table}

==> Tables/old_rectifying_result.tex <==
\begin{table*}[]
\centering
\footnotesize
\begin{tabular}{l|l|l|ccccc|ccccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}LLM\end{tabular}}} &
\multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Retriever\end{tabular}}} &
  \multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Method\end{tabular}}} &
  \multicolumn{5}{c}{MRPC} &
  \multicolumn{5}{c}{SST5} \\  
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{0} &
\multicolumn{1}{c}{0.1} &
\multicolumn{1}{c}{0.2} &
\multicolumn{1}{c}{0.3} &
\multicolumn{1}{c}{0.5} &
\multicolumn{1}{c}{0} &
\multicolumn{1}{c}{0.1} &
\multicolumn{1}{c}{0.2} &
\multicolumn{1}{c}{0.3} &
\multicolumn{1}{c}{0.5}\\ \midrule
\multirow{6}{*}{GPT-Neo} & 
\multirow{2}{*}{EPR} &
  w/o Rectification &
  \multicolumn{1}{c}{77.45} &
  \multicolumn{1}{c}{75.49} &
  \multicolumn{1}{c}{72.3} &
  \multicolumn{1}{c}{66.18} &
  \multicolumn{1}{c}{56.86} &
  \multicolumn{1}{c}{46.41} &
\multicolumn{1}{c}{42.6} &
\multicolumn{1}{c}{41.6} &
\multicolumn{1}{c}{37.69} &
\multicolumn{1}{c}{29.79} \\
 & & Rectification &
  \multicolumn{1}{c}{76.72} &
\multicolumn{1}{c}{76.72} &
\multicolumn{1}{c}{76.96} &
\multicolumn{1}{c}{76.47} &
\multicolumn{1}{c}{76.72} &
  \multicolumn{1}{c}{45.41} &
\multicolumn{1}{c}{44.87} &
\multicolumn{1}{c}{46.05} &
\multicolumn{1}{c}{42.96} &
\multicolumn{1}{c}{44.50}  \\ \cmidrule{2-13}
& \multirow{2}{*}{TopK-Bert} &
  w/o Rectification &
  \multicolumn{1}{c}{0} &
  \multicolumn{1}{c}{0} &
  \multicolumn{1}{c}{0} &
  \multicolumn{1}{c}{0} &
  \multicolumn{1}{c}{0} &
  \multicolumn{1}{c}{-} &
  \multicolumn{1}{c}{-} &
  \multicolumn{1}{c}{-} &
  \multicolumn{1}{c}{-} &
  \multicolumn{1}{c}{-}\\
 & &
  Rectification &
 \multicolumn{1}{c}{70.10} &
\multicolumn{1}{c}{68.63} &
\multicolumn{1}{c}{69.12} &
\multicolumn{1}{c}{69.85} &
\multicolumn{1}{c}{68.14} &
  \multicolumn{1}{c}{34.06} &
\multicolumn{1}{c}{34.24} &
\multicolumn{1}{c}{34.97} &
\multicolumn{1}{c}{36.78} &
\multicolumn{1}{c}{36.06} \\ \cmidrule{2-13}
& \multirow{2}{*}{Random} &
  w/o Rectification &
  \multicolumn{1}{c}{0} &
  \multicolumn{1}{c}{0} &
  \multicolumn{1}{c}{0} &
  \multicolumn{1}{c}{0} &
  \multicolumn{1}{c}{0} &
  \multicolumn{1}{c}{-} &
  \multicolumn{1}{c}{-} &
  \multicolumn{1}{c}{-} &
  \multicolumn{1}{c}{-} &
  \multicolumn{1}{c}{-}\\
 & & Rectification &
  \multicolumn{1}{c}{64.95} &
\multicolumn{1}{c}{63.73} &
\multicolumn{1}{c}{61.03} &
\multicolumn{1}{c}{64.95} &
\multicolumn{1}{c}{60.29} &
  \multicolumn{1}{c}{27.43} &
\multicolumn{1}{c}{26.98} &
\multicolumn{1}{c}{27.07} &
\multicolumn{1}{c}{26.25} &
\multicolumn{1}{c}{27.16} \\ \midrule
\multirow{6}{*}{LLaMA} & 
\multirow{2}{*}{EPR} &
  w/o Rectification &
  \multicolumn{1}{c}{0} &
  \multicolumn{1}{c}{0} &
  \multicolumn{1}{c}{0} &
  \multicolumn{1}{c}{0} &
  \multicolumn{1}{c}{0} &
  \multicolumn{1}{c}{-} &
  \multicolumn{1}{c}{-} &
  \multicolumn{1}{c}{-} &
  \multicolumn{1}{c}{-} &
  \multicolumn{1}{c}{-}\\
 & & Rectification &  
  \multicolumn{1}{c}{76.47} &
\multicolumn{1}{c}{76.72} &
\multicolumn{1}{c}{76.72} &
\multicolumn{1}{c}{76.72} &
\multicolumn{1}{c}{76.96} &
  \multicolumn{1}{c}{50.23} &
\multicolumn{1}{c}{50.95} &
\multicolumn{1}{c}{49.77} &
\multicolumn{1}{c}{48.96} &
\multicolumn{1}{c}{48.59} \\ \cmidrule{2-13}
& \multirow{2}{*}{TopK-Bert} &
  w/o Rectification &
  \multicolumn{1}{c}{0} &
  \multicolumn{1}{c}{0} &
  \multicolumn{1}{c}{0} &
  \multicolumn{1}{c}{0} &
  \multicolumn{1}{c}{0} &
  \multicolumn{1}{c}{-} &
  \multicolumn{1}{c}{-} &
  \multicolumn{1}{c}{-} &
  \multicolumn{1}{c}{-} &
  \multicolumn{1}{c}{-}\\
 & &
  Rectification &
  \multicolumn{1}{c}{69.61} &
\multicolumn{1}{c}{68.63} &
\multicolumn{1}{c}{69.36} &
\multicolumn{1}{c}{69.61} &
\multicolumn{1}{c}{68.38} &
\multicolumn{1}{c}{49.86} &
\multicolumn{1}{c}{49.86} &
\multicolumn{1}{c}{51.14} &
\multicolumn{1}{c}{51.04} &
\multicolumn{1}{c}{50.68} \\ \cmidrule{2-13}
& \multirow{2}{*}{Random} &
  w/o Rectification &
  \multicolumn{1}{c}{0} &
  \multicolumn{1}{c}{0} &
  \multicolumn{1}{c}{0} &
  \multicolumn{1}{c}{0} &
  \multicolumn{1}{c}{0} &
  \multicolumn{1}{c}{-} &
  \multicolumn{1}{c}{-} &
  \multicolumn{1}{c}{-} &
  \multicolumn{1}{c}{-} &
  \multicolumn{1}{c}{-}\\
 & & Rectification &
  \multicolumn{1}{c}{64.71} &
\multicolumn{1}{c}{63.48} &
\multicolumn{1}{c}{62.25} &
\multicolumn{1}{c}{65.20} &
\multicolumn{1}{c}{61.27} &
  \multicolumn{1}{c}{46.14} &
\multicolumn{1}{c}{45.32} &
\multicolumn{1}{c}{46.05} &
\multicolumn{1}{c}{44.41} &
\multicolumn{1}{c}{46.50}  \\ \bottomrule
\end{tabular}
\caption{SST5 results.}
\end{table*}
